Domain Generalization for Endoscopic Image Segmentation by Disentangling Style-Content Information and SuperPixel Consistency

Frequent monitoring is necessary to stratify individuals based on their likelihood of developing gastrointestinal (GI) cancer precursors. In clinical practice, white-light imaging (WLI) and complementary modalities such as narrow-band imaging (NBI) and fluorescence imaging are used to assess risk areas. However, conventional deep learning (DL) models show degraded performance due to the domain gap when a model is trained on one modality and tested on a different one. In our earlier approach, we used a superpixel-based method referred to as "SUPRA" to effectively learn domain-invariant information using color and space distances to generate groups of pixels. One of the main limitations of this earlier work is that the aggregation does not exploit structural information, making it suboptimal for segmentation tasks, especially for polyps and heterogeneous color distributions. Therefore, in this work, we propose an approach for style-content disentanglement using instance normalization and instance selective whitening (ISW) for improved domain generalization when combined with SUPRA. We evaluate our approach on two datasets: EndoUDA Barrett's Esophagus and EndoUDA polyps, and compare its performance with three state-of-the-art (SOTA) methods. Our findings demonstrate a notable enhancement in performance compared to both baseline and SOTA methods across the target domain data. Specifically, our approach exhibited improvements of 14%, 10%, 8%, and 18% over the baseline and three SOTA methods on the polyp dataset. Additionally, it surpassed the second-best method (EndoUDA) on the Barrett's Esophagus dataset by nearly 2%.

==> draft.tex <==
% https://drive.google.com/drive/u/0/folders/10-2_hmFWKoPmlNxqskvXiDZNx7yMjUMH


1. Intro

2. Metodos
    2.1. Generación @Ruben
        2.1.1. M2 
        2.1.2. Metricas (deepchecks)
        2.1.3. Imágenes para generar (Daudon) Menos imágenes
        No se ocuparon tantas imágenes. @Francisco
    2.2. Evaluation protocol @Francisco
        2.2.1. DL models
            2.2.1.1. Patch extraction (citar)
            2.2.1.1. Baseline (
            2.2.1.1. Two-step TL
        2.2.2. Metricas
        2.2.3. Dataset paches (Daudon, Jonathan, Ruben)
3. Resultados
    3.1. Generación (distribuciones deepcheks)
    3.2. Evaluacion DL (umaps): 
    3.3. Comparativa* 
        Entrada para cada vista - M1 - m2
 
4. Discusión
5. Conclusiones



todo; Autores una línea. 






Figura. @Francisco
a. Dataset real (2x6). 
b. Dataset generadas (2x6)

Tabla. Dataset @Francisco
a. Real

Figura. Pipeline. @Ruben

Figura. 






%% Titulo + Abstract + intro (una pagina)

Advanced Medical Imaging using AI/DL

Endoscopia y uretrotsicpoia que hay u8n gran interes de desarrollar herramientas de CAD: claisisfacion,d eteccio y segmentacion y ha bido algunos avances significativos

Sin embargo uno de los principales problemas es la falta de datos, tanto para entrenar modelos pero tambien datos sintéticos que simulen diferenrtes condiciones de adquisición y diferentes tipos de endoscopio

En el contexto de ureteroscopia, hay un gran intereses en la identificación automática de calculos renales: el MCA es una herramienta ampliamente utilizada, pero el problema adicionales a los otros menciodaods es que hay una gran imblance de clases, debido a que ciertos tipos de calculos renales son pocos comunes, lo cual exacerba o hace mas complejo el entrenamiento y validacion de modelo

En ese sentido, en este trabajo proponemos un estudio pre-liminar para la generación de imagees sinteticas de calculos renales a partir de un dataset pre-existente, con XYZ caracteristcas (como su capturo y que tipos de imágenes son)

El primer objetivo es la generación de imágenes altamente similares en un datast ex-vivo, para posteriormente hacer image translation y proceder a la generación de imágenes endoscopia a partir imágenes ex-vivo.Posteriormente se abordar la generación de imágenes realistas.

Para tal fin se utilizo el modelo generativo basado en el trabajo de los autores, etc.

Los resultados obtenidos de este protocolo experimentas son prometedores, pues permiten general imágenes altamente realistas que serán validados por expertos en el campo de la MCA


Motivation → el interes del MCA y lun poco sobre las clases de cálculos renales que existen

(media página)

Datasets (media pagina)

Dataset de Daudon

Methods (1 pagina)

Modelo utilizado M2

Entrenamiento

Generación → FID y validacion por expertos y por modelos pre-entrenados
img generadas
Validación -> DL baseline/2step
umaps
Resultados (1 pagina)

Image de las imagenes generadas, alguna tabla, discusion/conclusiones

